PanoEnv: Exploring 3D Spatial Intelligence in Panoramic Environments with Reinforcement Learning

360 panoramic images are increasingly used in virtual reality, autonomous driving, and robotics for holistic scene understanding. However, current Vision-Language Models (VLMs) struggle with 3D spatial reasoning on Equirectangular Projection (ERP) images due to geometric distortion and limited 3D supervision. We introduce PanoEnv, a large-scale VQA benchmark built from synthetic 3D environments, containing 14.8K questions across five categories (e.g., relative position, volume comparison) grounded in accurate 3D annotations including depth, segmentation, and bounding boxes. Benchmarking 14 state-of-the-art VLMs reveals limited 3D understanding, achieving only 49.34% overall accuracy and 8.36% on open-ended (OE) questions. To enhance 3D reasoning, we propose a reinforcement learning post-training framework based on Group Relative Policy Optimization (GRPO) with a ground-truth-guided reward that incorporates five geometry-aware strategies such as distance tolerance and spatial consistency. A two-stage curriculum further mitigates catastrophic forgetting: Stage 1 trains on structured tasks (true/false and multiple choice), and Stage 2 fine-tunes on mixed open-ended data to improve generalization. Our 7B model achieves new state-of-the-art performance, improving overall accuracy to 52.93% (+3.59%) and open-ended accuracy to 14.83% while maintaining structured-task performance. It also achieves top semantic evaluation scores (Q-Score 6.24, P-Score 5.95), surpassing 32B models. These results demonstrate that PanoEnv-QA and our curriculum-based RL framework effectively instill 3D spatial intelligence in VLMs for omnidirectional perception.

==> tables/ablation_components.tex <==
\begin{table*}[htbp]
\centering
\Large
\caption{\textbf{Ablation on Components of the Pipeline.} We present an ablation study on components of the pipeline using the EgoTextVQA benchmark. ``ACC" refers to Accuracy. v5: all components.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc} % 15 列
\toprule
\multicolumn{15}{c}{\Large\textbf{Ablation on the Maximum Number of Detected Objects Parameter on EgoTextVQA-Indoor}} \\ % ← 改为 15 列
\midrule
\multirow{2}{*}{\textbf{Component}} &
\multicolumn{2}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Hands-on}} &
\multicolumn{2}{c|}{\textbf{Kitchen}} &
\multicolumn{2}{c|}{\textbf{Shopping}} &
\multicolumn{2}{c|}{\textbf{Gameplay}} &
\multicolumn{2}{c|}{\textbf{Book-Related}} &
\multicolumn{2}{c}{\textbf{Others}} \\ 
\cmidrule(lr){2-15}
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} \\ 
\midrule
v0 Original              & 31.20 & 2.24 & 31.81 & 2.27 & 26.87 & 2.07 & 24.58 & 1.97 & 41.53 & 2.65 & 36.02 & 2.46 & 24.88 & 1.98 \\
v1 + Region           & 31.38 & 2.25 & 31.13 & 2.24 & 25.97 & 2.03 & 27.09 & 2.07 & 42.52 & 2.68 & 35.29 & 2.40 & 25.87 & 2.02 \\
v2 + Depth        & 33.41 & 2.32 & 33.57 & 2.33 & 27.46 & 2.09 & 29.05 & 2.14 & 44.52 & 2.76 & 36.53 & 2.44 & 28.86 & 2.14 \\
v3 + Text & 33.54 & 2.33 & 33.43 & 2.33 & 28.06 & 2.11 & 28.21 & 2.11 & 45.51 & 2.79 & 37.15 & 2.46 & 28.86 & 2.14 \\
\rowcolor{gray!15}
v4 + Organize Information in Graph            & 33.74 & 2.34 & 33.86 & 2.35 & 28.96 & 2.15 & 28.49 & 2.12 & 45.00 & 2.78 & 36.84 & 2.45 & 28.86 & 2.14 \\
\bottomrule
\end{tabular}
}
\label{tab:ablation_components}
\end{table*}


==> tables/ablation_num.tex <==
\begin{table*}[htbp]
\centering
\Large
\caption{\textbf{Ablation on the Maximum Number of Detected Objects Parameter.} We present an ablation study on the maximum number of detected objects hyperparameter using the EgoTextVQA benchmark, varying its value to 2, 4, 6, 8, and 10. The results indicate that a setting of 4 for \textit{maximum number} shows the best performance. ``ACC" refers to Accuracy, and ``Num. Object" to the maximum number of objects we detect.}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc|cc} % 15 列
\toprule
\multicolumn{15}{c}{\Large\textbf{Ablation on the Maximum Number of Detected Objects Parameter on EgoTextVQA-Indoor}} \\ % ← 改为 15 列
\midrule
\multirow{2}{*}{\textbf{Num. Object}} &
\multicolumn{2}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Hands-on}} &
\multicolumn{2}{c|}{\textbf{Kitchen}} &
\multicolumn{2}{c|}{\textbf{Shopping}} &
\multicolumn{2}{c|}{\textbf{Gameplay}} &
\multicolumn{2}{c|}{\textbf{Book-Related}} &
\multicolumn{2}{c}{\textbf{Others}} \\ 
\cmidrule(lr){2-15}
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} 
 & \textbf{ACC} & \textbf{Score} \\ 
\midrule
Value = 2  & 32.91 & 2.30 & 33.29 & 2.32 & 28.06 & 2.11 & 27.65 & 2.09 & 43.85 & 2.73 & 36.22 & 2.43 & 27.36 & 2.08 \\
\rowcolor{gray!15}
Value = 4  & 33.74 & 2.34 & 33.86 & 2.35 & 28.96 & 2.15 & 28.49 & 2.12 & 45.00 & 2.78 & 36.84 & 2.45 & 28.86 & 2.14 \\
Value = 6  & 33.32 & 2.32 & 33.00 & 2.32 & 28.36 & 2.12 & 28.77 & 2.13 & 43.85 & 2.73 & 36.53 & 2.44 & 29.85 & 2.18 \\
Value = 8  & 33.41 & 2.32 & 33.14 & 2.32 & 28.66 & 2.14 & 28.49 & 2.12 & 44.19 & 2.74 & 36.53 & 2.44 & 29.85 & 2.18 \\
Value = 10 & 33.45 & 2.33 & 33.00 & 2.32 & 29.25 & 2.16 & 28.49 & 2.12 & 44.52 & 2.75 & 36.53 & 2.44 & 29.35 & 2.16 \\
\bottomrule
\end{tabular}
}
\label{tab:ablation_num}
\end{table*}


==> tables/egotextvqa_result.tex <==
% \usepackage{caption}
% \usepackage{subcaption} % ← 加入导言区

\begin{table*}[htbp]
\centering
\Large
\caption{\textbf{Evaluation Results on the EgoTextVQA Benchmark} for both indoor and outdoor settings. ``ACC'' refers to Accuracy, and ``Int. Reasoning"to Intention Reasoning. Gains relative to the SoTA (Qwen2.5-VL) model are indicated in \textcolor{violet!85}{violet}, while reductions are highlighted using \textcolor{red!20!green!20!blue!50}{blue}.}

% ===== 上半部分：Indoor =====
\begin{subtable}{\textwidth}
\centering
\caption{\textbf{EgoTextVQA-Indoor Results}}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cc|cc|cc|cc|cc|cc}
\midrule
\multicolumn{17}{c}{\Large\textbf{EgoTextVQA-Indoor}} \\
\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Hands-on}} &
\multicolumn{2}{c|}{\textbf{Kitchen}} &
\multicolumn{2}{c|}{\textbf{Shopping}} &
\multicolumn{2}{c|}{\textbf{Gameplay}} &
\multicolumn{2}{c|}{\textbf{Book-Related}} &
\multicolumn{2}{c}{\textbf{Others}} \\
\cmidrule(lr){2-17}
 & \textbf{ACC} & \textbf{$\Delta$ACC} & \textbf{Score} & \textbf{$\Delta$Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} \\
\midrule
InstructBLIP & 28.09 & \downx{3.11} & 2.12 & \downx{0.12} & 26.26 & 2.05 & 25.45 & 2.01 & 26.54 & 2.04 & 37.54 & 2.49 & 30.96 & 2.24 & 22.89 & 1.92 \\
Emu3 & 9.16 & \downx{22.04} & 1.37 & \downx{0.87} & 8.88 & 1.35 & 12.24 & 1.49 & 6.98 & 1.29 & 9.30 & 1.37 & 10.52 & 1.42 & 6.47 & 1.26 \\
LLaVA-NeXT & 28.35 & \downx{2.85} & 2.13 & \downx{0.11} & 27.98 & 2.11 & 24.48 & 1.97 & 26.82 & 2.06 & 36.54 & 2.46 & 30.34 & 2.20 & 23.38 & 1.94 \\
InternVL2 & 28.52 & \downx{2.68} & 2.12 & \downx{0.12} & 27.65 & 2.09 & 23.88 & 1.93 & 23.74 & 1.95 & 38.21 & 2.51 & 32.51 & 2.29 & 26.87 & 2.03 \\
Qwen2-VL & 28.97 & \downx{2.23} & 2.15 & \downx{0.09} & 28.51 & 2.12 & 23.28 & 1.91 & 23.46 & 1.94 & 39.87 & 2.58 & 33.44 & 2.33 & 26.37 & 2.04 \\
Qwen2.5-VL & 31.20 & \baseval{-0.00} & 2.24 & \baseval{-0.00} & 31.81 & 2.27 & 26.87 & 2.07 & 24.58 & 1.97 & 41.53 & 2.65 & 36.02 & 2.46 & 24.88 & 1.98 \\ \midrule
\rowcolor{gray!15}
Ours & \textbf{33.74} & \upx{2.54} & \textbf{2.34} & \upx{0.10} & \textbf{33.86} & \textbf{2.35} & \textbf{28.96} & \textbf{2.15} & \textbf{28.49} & \textbf{2.12} & \textbf{45.00} & \textbf{2.78} & \textbf{36.84} & 2.45 & \textbf{28.86} & \textbf{2.14} \\
\midrule
\end{tabular}
}
\end{subtable}

\vspace{1.5em} % ← 调整上下间距

% ===== 下半部分：Outdoor =====
\begin{subtable}{\textwidth}
\centering
\caption{\textbf{EgoTextVQA-Outdoor Results}}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccc|cc|cc|cc|cc|cc}
\midrule
\multicolumn{15}{c}{\Large\textbf{EgoTextVQA-Outdoor}} \\
\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Location}} &
\multicolumn{2}{c|}{\textbf{Direction}} &
\multicolumn{2}{c|}{\textbf{Description}} &
\multicolumn{2}{c|}{\textbf{Int. Reasoning}} &
\multicolumn{2}{c}{\textbf{Others}} \\
\cmidrule(lr){2-15}
 & \textbf{ACC} & \textbf{$\Delta$ACC} & \textbf{Score} & \textbf{$\Delta$Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} \\
\midrule
InstructBLIP & 21.07 & \downx{4.16} & 1.84 & \downx{0.16} & 14.29 & 1.56 & 30.25 & 2.22 & 20.99 & 1.83 & 22.14 & 1.91 & 24.74 & 1.99 \\
Emu3 & 5.71 & \downx{19.52} & 1.24 & \downx{0.76} & 5.51 & 1.22 & 10.08 & 1.43 & 3.46 & 1.14 & 5.29 & 1.22 & 3.66 & 1.13 \\
LLaVA-NeXT & 21.00 & \downx{4.23} & 1.84 & \downx{0.16} & 13.36 & 1.53 & 30.99 & 2.26 & 21.12 & 1.84 & 22.02 & 1.90 & 26.32 & 2.05 \\
InternVL2 & 23.97 & \downx{1.26} & 1.95 & \downx{0.05} & 18.54 & 1.73 & 31.93 & 2.28 & 26.10 & 2.03 & 18.94 & 1.78 & \textbf{32.98} & \textbf{2.29} \\
Qwen2-VL & 24.92 & \downx{0.31} & 1.99 & \downx{0.01} & 20.00 & 1.79 & 32.67 & 2.32 & 26.24 & 2.04 & 21.03 & 1.85 & 31.94 & 2.23 \\
Qwen2.5-VL & 25.23 & \baseval{-0.00} & 2.00 & \baseval{-0.00} & 18.60 & 1.73 & 34.98 & \textbf{2.42} & 27.33 & 2.07 & 21.53 & 1.87 & 29.32 & 2.17 \\
\rowcolor{gray!15}
Ours & \textbf{27.43} & \upx{2.20} & \textbf{2.09} & \upx{0.09} & \textbf{20.86} & \textbf{1.82} & \textbf{37.71} & 2.25 & \textbf{28.41} & \textbf{2.12} & \textbf{24.97} & \textbf{2.02} & 31.41 & 2.24 \\
\midrule
\end{tabular}
}
\end{subtable}

\label{tab:egotextvqa_combined}
\end{table*}


==> tables/egotextvqa_result_indoor.tex <==
% 自定义符号与颜色
\newcommand{\upx}[1]{\textcolor{violet!85}{$\uparrow$#1}}
\newcommand{\downx}[1]{\textcolor{red!20!green!20!blue!50}{$\downarrow$#1}}
\newcommand{\baseval}[1]{\textcolor{gray!85}{#1}}

\begin{table}[htbp]
\centering
\Large % ← 字号变大
\caption{\textbf{Evaluation Results on the EgoTextVQA Benchmark} of baselines and our ESA on the indoor setting. ``ACC" refers to Accuracy.
To facilitate a direct comparison of performance, we set the performance of the SoTA (Qwen2.5-VL) model as \baseval{-0.00}. 
Gains relative to the SoTA model are indicated in \textcolor{violet!85}{violet}, while reductions are highlighted using \textcolor{red!20!green!20!blue!50}{blue}.}
\resizebox{\columnwidth}{!}{ % ← 宽度放大到 105%
\begin{tabular}{l|cccc|cc|cc|cc|cc|cc|cc}
\midrule
\multicolumn{17}{c}{\Large\textbf{EgoTextVQA-Indoor}} \\ % ← 顶部标题，字体同步放大
\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Hands-on}} &
\multicolumn{2}{c|}{\textbf{Kitchen}} &
\multicolumn{2}{c|}{\textbf{Shopping}} &
\multicolumn{2}{c|}{\textbf{Gameplay}} &
\multicolumn{2}{c|}{\textbf{Book-Related}} &
\multicolumn{2}{c}{\textbf{Others}} \\ 
\cmidrule{2-17}
 & \textbf{ACC} & \textbf{$\Delta$ACC} & \textbf{Score} & \textbf{$\Delta$Score} 
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} \\ 
\midrule
InstructBLIP & 28.09 & \downx{3.11} & 2.12 & \downx{0.12} & 26.26 & 2.05 & 25.45 & 2.01 & 26.54 & 2.04 & 37.54 & 2.49 & 30.96 & 2.24 & 22.89 & 1.92 \\
Emu3 & 9.16 & \downx{22.04} & 1.37 & \downx{0.87} & 8.88 & 1.35 & 12.24 & 1.49 & 6.98 & 1.29 & 9.30 & 1.37 & 10.52 & 1.42 & 6.47 & 1.26 \\
LLaVA-NeXT & 28.35 & \downx{2.85} & 2.13 & \downx{0.11} & 27.98 & 2.11 & 24.48 & 1.97 & 26.82 & 2.06 & 36.54 & 2.46 & 30.34 & 2.20 & 23.38 & 1.94 \\
InternVL2 & 28.52 & \downx{2.68} & 2.12 & \downx{0.12} & 27.65 & 2.09 & 23.88 & 1.93 & 23.74 & 1.95 & 38.21 & 2.51 & 32.51 & 2.29 & 26.87 & 2.03 \\
Qwen2-VL & 28.97 & \downx{2.23} & 2.15 & \downx{0.09} & 28.51 & 2.12 & 23.28 & 1.91 & 23.46 & 1.94 & 39.87 & 2.58 & 33.44 & 2.33 & 26.37 & 2.04 \\
Qwen2.5-VL & 31.20 & \baseval{-0.00} & 2.24 & \baseval{-0.00} & 31.81 & 2.27 & 26.87 & 2.07 & 24.58 & 1.97 & 41.53 & 2.65 & 36.02 & \textbf{2.46} & 24.88 & 1.98 \\
\rowcolor{gray!15}
Ours & \textbf{33.74} & \upx{2.54} & \textbf{2.34} & \upx{0.10} & \textbf{33.86} & \textbf{2.35} & \textbf{28.96} & \textbf{2.15} & \textbf{28.49} & \textbf{2.12} & \textbf{45.00} & \textbf{2.78} & \textbf{36.84} & 2.45 & \textbf{28.86} & \textbf{2.14} \\
\midrule
\end{tabular}
}
\label{tab:egotextvqa_result_indoor}
\end{table}


==> tables/egotextvqa_result_outdoor.tex <==
% 自定义符号与颜色
% \newcommand{\upx}[1]{\textcolor{violet!85}{$\uparrow$#1}}
% \newcommand{\downx}[1]{\textcolor{red!20!green!20!blue!50}{$\downarrow$#1}}
% \newcommand{\baseval}[1]{\textcolor{gray!85}{#1}}

\begin{table}[htbp]
\centering
\label{tab:egotextvqa_result_outdoor}
\Large
\caption{\textbf{Evaluation Results on the EgoTextVQA Benchmark} of baselines and our ESA on the outdoor setting. ``ACC" refers to Accuracy and ``Int. Reasoning" to Intention Reasoning.
To facilitate a direct comparison of performance, we set the performance of the SoTA (Qwen2.5-VL) model as \baseval{-0.00}. 
Gains relative to the SoTA model are indicated in \textcolor{violet!85}{violet}, while reductions are highlighted using \textcolor{red!20!green!20!blue!50}{blue}.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccc|cc|cc|cc|cc|cc}
\midrule
\multicolumn{15}{c}{\Large\textbf{EgoTextVQA-Outdoor}} \\ % 顶部标题
\midrule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{c|}{\textbf{Average}} &
\multicolumn{2}{c|}{\textbf{Location}} &
\multicolumn{2}{c|}{\textbf{Direction}} &
\multicolumn{2}{c|}{\textbf{Description}} &
\multicolumn{2}{c|}{\textbf{Int. Reasoning}} &
\multicolumn{2}{c}{\textbf{Others}} \\ 
\cmidrule{2-15}
 & \textbf{ACC} & \textbf{$\Delta$ACC} & \textbf{Score} & \textbf{$\Delta$Score} 
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score}
 & \textbf{ACC} & \textbf{Score} & \textbf{ACC} & \textbf{Score} \\ 
\midrule
InstructBLIP & 21.07 & \downx{4.16} & 1.84 & \downx{0.16} & 14.29 & 1.56 & 30.25 & 2.22 & 20.99 & 1.83 & 22.14 & 1.91 & 24.74 & 1.99 \\
Emu3 & 5.71 & \downx{19.52} & 1.24 & \downx{0.76} & 5.51 & 1.22 & 10.08 & 1.43 & 3.46 & 1.14 & 5.29 & 1.22 & 3.66 & 1.13 \\
LLaVA-NeXT & 21.00 & \downx{4.23} & 1.84 & \downx{0.16} & 13.36 & 1.53 & 30.99 & 2.26 & 21.12 & 1.84 & 22.02 & 1.90 & 26.32 & 2.05 \\
InternVL2 & 23.97 & \downx{1.26} & 1.95 & \downx{0.05} & 18.54 & 1.73 & 31.93 & 2.28 & 26.10 & 2.03 & 18.94 & 1.78 & \textbf{32.98} & \textbf{2.29} \\
Qwen2-VL & 24.92 & \downx{0.31} & 1.99 & \downx{0.01} & 20.00 & 1.79 & 32.67 & 2.32 & 26.24 & 2.04 & 21.03 & 1.85 & 31.94 & 2.23 \\
Qwen2.5-VL & 25.23 & \baseval{-0.00} & 2.00 & \baseval{-0.00} & 18.60 & 1.73 & 34.98 & \textbf{2.42} & 27.33 & 2.07 & 21.53 & 1.87 & 29.32 & 2.17 \\
\rowcolor{gray!15}
Ours & \textbf{27.43} & \upx{2.20} & \textbf{2.09} & \upx{0.09} & \textbf{20.86} & \textbf{1.82} & \textbf{37.71} & 2.25 & \textbf{28.41} & \textbf{2.12} & \textbf{24.97} & \textbf{2.02} & 31.41 & 2.24 \\
\midrule
\end{tabular}
}
\label{tab:egotextvqa_result_outdoor}
\end{table}

